Draft-based Approximate Inference for LLMs

Optimizing inference for long-context large language models (LLMs) is increasingly important due to the quadratic compute and linear memory cost of Transformers. Existing approximate inference methods, including key-value (KV) cache dropping, sparse attention, and prompt compression, typically rely on coarse predictions of token or KV pair importance. We unify and extend recent work by introducing a framework for approximate LLM inference that leverages small draft models to more accurately predict token and KV pair importance. We provide novel theoretical and empirical analyses justifying lookahead-based importance estimation techniques. Within this framework, we present: (i) SpecKV, the first method to use lookahead with a small draft model to enable precise KV cache dropping; (ii) SpecPC, which leverages draft model attention activations to identify and discard less important prompt tokens; and (iii) SpecKV-PC, a cascaded compression strategy combining both techniques. Extensive experiments on long-context benchmarks demonstrate that our methods consistently achieve higher accuracy than existing baselines while retaining the same efficiency gains in memory usage, latency, and throughput.

==> src/attn_corr_fig.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/attn_corr_main/attn_corr_llama_mean_2_0.5.pdf}
         \caption{Mean aggregation \kg{Importance score correlation}}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/attn_corr_main/attn_corr_llama_max_1_0.05.pdf}
         \caption{Max aggregation \kg{R2 vs downstream}}
     \end{subfigure}
    % \caption{Correlation of attention activations between Llama-3.2-1B (draft) and Llama-3.1-8B (target)  models for 45 examples from the RULER (16K)~\cite{ruler} benchmark (five examples from each of nine tasks). For each model, attention maps are aggregated over all layers, heads, and queries, using either the mean or the maximum value per key. Each point plots the aggregated activation of a key in the draft model against that in the target model. Both mean (a) and max (b) aggregation methods show that the draft and target models exhibit highly correlated attention activations.}
    \caption{Correlation of attention activations between Llama-3.2-1B (draft) and Llama-3.1-8B (target) on 45 RULER (16K)~\cite{ruler} examples (five per each of nine tasks). Attention maps are aggregated across layers, heads, and queries using mean or max per key. Each point plots a key’s activation in the draft versus target model. Both aggregation methods ((a) mean, (b) max) reveal strong correlations. \kg{change to importance scores, also in the appendix?}}
    \label{fig:attn_corr}
\end{figure}
